Can LLMs Understand Time Series Anomalies?

Large Language Models (LLMs) have gained popularity in time series forecasting, but their potential for anomaly detection remains largely unexplored. Our study investigates whether LLMs can understand and detect anomalies in time series data, focusing on zero-shot and few-shot scenarios. Inspired by conjectures about LLMs' behavior from time series forecasting research, we formulate key hypotheses about LLMs' capabilities in time series anomaly detection. We design and conduct principled experiments to test each of these hypotheses. Our investigation reveals several surprising findings about LLMs for time series: (1) LLMs understand time series better as images rather than as text, (2) LLMs do not demonstrate enhanced performance when prompted to engage in explicit reasoning about time series analysis. (3) Contrary to common beliefs, LLMs' understanding of time series does not stem from their repetition biases or arithmetic abilities. (4) LLMs' behaviors and performance in time series analysis vary significantly across different models. This study provides the first comprehensive analysis of contemporary LLM capabilities in time series anomaly detection. Our results suggest that while LLMs can understand trivial time series anomalies, we have no evidence that they can understand more subtle real-world anomalies. Many common conjectures based on their reasoning capabilities do not hold. All synthetic dataset generators, final prompts, and evaluation scripts have been made available in https://github.com/rose-stl-lab/anomllm.

==> secs/draft.tex <==

% \subsection{Real-World Dataset}

% \paragraph{Server Machine Dataset (SMD).}

% SMD is a 5-week-long dataset collected from 28 server machines at a large Internet company. It includes data from 38 different sensors or metrics per machine, which monitor various aspects of the server’s operation, such as CPU load, network usage, and memory usage. The data was recorded at 1-minute intervals, and domain experts have labeled anomalies and their anomalous dimensions in the SMD testing set. The research outlined in employed this dataset for its analysis.

% \paragraph{Yahoo S5.}

% The Yahoo S5 dataset is a labeled open dataset for anomaly detection released by Yahoo Lab. Part of the time series is synthetic (i.e., simulated). In contrast, the other part comes from the real traffic of Yahoo services. The anomaly points in the simulated curves are algorithmically generated, and those in the real-traffic curves are labeled by editors manually. The dataset was prominently featured in the experimental findings of paper.


% \subsection{Synthetic Dataset}

% The synthetic dataset used in this anomaly detection study comprises seven distinct subsets, each containing 400 time series. These subsets are designed to simulate various types of anomalies commonly encountered in real-world data: point, range, trend, frequency, and their noisy counterparts (noisy-point, noisy-trend, and noisy-freq). Each subset is crafted to represent specific patterns and anomalies, allowing for a comprehensive evaluation of anomaly detection algorithms across diverse scenarios.

% The datasets exhibit varying characteristics in terms of anomaly prevalence and structure. For instance, the trend and noisy-trend datasets have the highest percentage of time series without anomalies (57.50\% and 60.50\% respectively), while the freq and noisy-freq datasets have the lowest (10.00\% and 12.75\%). The average anomaly ratio across all datasets ranges from 0.0236 to 0.0377, indicating a relatively low but consistent presence of anomalies. The nature of anomalies varies significantly among the datasets, with some featuring short, frequent anomalies (e.g., freq dataset with an average of 2.16 anomalies per series and average length of 15.77), while others contain longer, less frequent anomalies (e.g., trend dataset with an average of 0.42 anomalies per series and average length of 88.61).

% The generation settings for each dataset type are tailored to produce specific normal and abnormal patterns. For example, the trend dataset features a steady increasing trend from -1 to 1 as normal data, with anomalies manifesting as sudden changes in trend or speed. The point dataset, on the other hand, presents a periodic sine wave as normal data, with anomalies appearing as noisy and unpredictable deviations. More detailed parameters and descriptions for each dataset type, including the noisy variants, are provided in the appendix. These carefully designed datasets aim to challenge and evaluate the robustness of anomaly detection algorithms across a wide range of scenarios.

% \subsection{Draft}

% The following hypotheses represent a synthesis of existing literature, prevailing assumptions in the field, and our own insights into LLM behavior. Many of these hypotheses stem from previous work, some of which may have been proposed without rigorous empirical validation. Others represent commonly held beliefs in the AI community that warrant closer examination. By subjecting these hypotheses to our comprehensive evaluation framework, we aim to:

% Validate or challenge assumptions made in previous studies
% Provide empirical evidence for claims that have been largely theoretical
% Uncover potential biases or limitations in current thinking about LLMs and time series analysis
% Identify areas where LLMs may surpass or fall short of human-like reasoning in anomaly detection
% Through this approach, we not only test specific hypotheses but also contribute to a more nuanced understanding of LLM capabilities in time series analysis. Each hypothesis below addresses a critical aspect of LLM performance, ranging from multimodal processing to inherent biases:

% This transition acknowledges the diverse origins of the hypotheses, highlights the potential for some to be based on unverified assumptions, and emphasizes the importance of rigorous testing. It also sets the stage for a critical examination of each hypothesis using your evaluation framework.

% \subsection*{Claims in the paper}
% The remarkable progress in large language models (LLMs) has demonstrated their ability to comprehend and generate human-like text. However, their effectiveness in understanding and detecting anomalies in time series data remains questionable. Recent studies have highlighted the limitations of LLMs in handling \textbf{long, context-rich datasets}, particularly in time series related tasks.

% We argue that the direct use of time series data as text input for LLMs may be a wrong approach to understanding time series. Instead, we propose that LLM with multimodality, especially by converting time series data into images, are key to leverage the extrapolation abilities of foundational models to overcome these limitations. The idea of converting time series data into images isn't new and is used in methods like Gramian Angular Fields (GAF) or Recurrence Plots. This integration could potentially offset some of the limitations of LLMs in handling raw \textbf{numeric time series data} by utilizing spatial pattern recognition ability of the pre-trained vision models \citep{tan2024are}.

% We contend that the process of identifying patterns in images---such as pixel frequency, density, and trends---is more akin to detecting patterns in time series data than it is to identifying anomalies in text. This is primarily because time series analysis, like image pattern recognition, involves assessing visual and sequential consistencies, whereas text anomaly detection typically focuses on deviations in language structure and syntax, which do not directly correlate with numerical or visual pattern recognition.

% We aim to investigate the effectiveness of using LLMs with vision capabilities for time series anomaly detection. By comparing this approach with traditional time series anomaly detection methods and evaluating its performance across different types of time series data and anomaly scenarios, we seek to contribute to the advancement of anomaly detection techniques in the era of large language models. Our goal is not to propose a new approach but to critically examine and validate the multimodal pathway for LLMs to understand time series anomalies effectively.


% \subsection*{Meaningful question}
% \begin{enumerate}
%     \item \textbf{Why extrapolation?}
%     \begin{enumerate}
%         \item The paper directly assumes LLMs can perform extrapolation on time series.
%         \item Why it is a given that LLMs can do ``simple arithmetic operations''?
%     \end{enumerate}
%     \item \textbf{Too simple?}
%     \begin{enumerate}
%         \item the proposed method is effective only for some simple time series data (such as obvious periodicity or trend), but not for some more complex time series data (such as wooly or HeartRate).
%         \item All these are fixed functions that have no dependence on the previously occurring values. Something that may be more interesting is e.g. the Fibonacci sequence.
%         \item You generalize this interesting feature they observed on toyish examples as a general feature of LLM.
%     \end{enumerate}
%     \item \textbf{What does ``simple'' mean?}
%     \begin{enumerate}
%         \item Although these are simple to us, they may be complicated functions to learn in the embedding space, and they depend on the tokenization used.
%     \end{enumerate}
%     \item \textbf{Questionable claims?}
%     \begin{enumerate}
%         \item Time series are relatively unstructured.
%         \item uncertainty quantification for time series also tends to be domain-specific and ad hoc
%     \end{enumerate}
% \end{enumerate}

% \subsection*{Question needed to handle with care}
% \begin{itemize}
%     \item \textbf{Numerical performance} would not be strong enough.
%     \begin{itemize}
%         \item Since you do not answer the research question, your paper is a feature / prompt engineering method paper, so you need numerical result
%         \item Since your dataset is simple, so you need numerical result on real-world dataset to show it generalize to real-world settings.
%     \end{itemize}
%     \item \textbf{There are already papers doing this.}
%     \begin{itemize}
%         \item There are already papers showing that LLM approaches generalize better then regular approaches.
%     \end{itemize}
%     \item \textbf{Baselines are lacking.}
%     \begin{itemize}
%         \item Where is Informer, Autoformer, and FEDformer?
%     \end{itemize}
% \end{itemize}



% \citet{zhu2024llms} shows the zero-shot learning abilities of VLM for anomaly detecgtion. They  propose a run-time prompt adaptation strategy, which first generates informative anomaly prompts to leverage the capabilities of a large language model (LLM). This strategy is enhanced by a contextual scoring mechanism for per-image anomaly prompt adaptation and cross-semantic ambiguity mitigation. 

% \cite{zanella2024harnessing} based on CLIP

% Qwen-VL. --- always gives the same anomaly input (max), pro (smaller) model.


% TS-Bert \citep{paszynski_ts-bert_2021} adapts the BERT model \cite{devlin_bert_2019} for time series anomaly detection by leveraging the pre-training and fine-tuning paradigm. Unlike methods that directly feed time series data as text into large language models, TS-Bert introduces a preprocessing step to normalize and discretize the values, making them compatible with BERT's input format. The pre-training phase involves Masked LM and Next Sentence Prediction tasks, which learn the intrinsic patterns and dependencies in time series data. During fine-tuning, TS-Bert is adapted to the specific anomaly detection task using generated pseudo-labels from an unsupervised method, SR \citep{ren_time-series_2019}. The paper also highlights modifications made to the BERT architecture to better suit time series data, such as handling long-distance dependencies and adjusting the input representation to capture the temporal nature of the data.




This question is not as straightforward as the empirical performance of state-of-the-art algorithms might suggest, since those results were challenged by simplified models, and those models do not receive time series data in a human-readable format. 

Recently, there has been a surge of Large Language Model~(LLM) applications to time series, mostly time-series forecasting and, to a much lesser extent, anomaly detection. Popular LLM-based time series analysis methods assume that LLM can understand and reason about time series data. However, do language models actually understand time series pattern, and is their inference benefited from their pretrained reasoning power? The answer is not as straightforward as empirical performance of SOTA algorithms suggest, as they usually do not receive time series as human readable format and are challenged by simplified models. We look into the black box of LLM-based time series analysis methods by focusing on the often overlooked time series anomaly detection task. After a series of ablation studies, we find that while LLM can ``understand'' simple time series anomalies, their ability to understand is highly relevant to their reasoning power and the modality they receive the time series. We find that some common assumptions on how LLM understand time series data are not true, different family of LLMs have different understanding of time series data, and LLMs have a preference for certain types of time series anomalies. Our work is the first to systematically examine large language models' anomaly detection ability on time series data. This work suggests that while using LLMs for analyzing time series is well motivated, they may not be as interpretable as they seem. Additionally, we introduce a new benchmark, TimeSeriesAD, for evaluating the text-based and visually grounded time series pattern understanding ability of LLMs.



Recent years have seen a surge in Large Language Model~(LLM) applications for time series analysis, primarily in forecasting and, to a lesser extent, anomaly detection. These LLM-based methods often assume that language models can understand and reason about time series data. However, do language models actually ``understand'' time series patterns? This question is not as straightforward as the empirical performance of state-of-the-art algorithms might suggest, since those results were challenged by simplified models, and those models do not receive time series data in a human-readable format. Our study delves into the black box of LLM-based time series analysis, focusing on the often-overlooked task of time series anomaly detection. Through a series of ablation studies, we find that while LLM can understand simple time series anomalies, their ability to understand is closely tied to their reasoning power and the modality they receive the time series. We find that some common assumptions on how LLM understand time series data are not true, different families of LLMs exhibit varying ways of comprehension, and LLMs show preferences for certain types of time series anomalies. Our work represents the first systematic examination of anomaly detection capabilities in time series data. This research suggests that while using LLMs for time series analysis is well-motivated, they may not be as interpretable as they initially appear. To further advance this field, we introduce TimeSeriesAD, a new benchmark for evaluating LLMs' text-based and visually grounded understanding of time series patterns.





Our findings have important implications for the development and application of LLM-based time series analysis methods, highlighting the need for careful consideration of model limitations and potential biases in their interpretation of time series data.









we investigate whether LLMs truly comprehend time series patterns and if their inference benefits from pretrained reasoning capabilities. Our findings reveal that while LLMs can "understand" simple time series anomalies, their comprehension is closely tied to their reasoning power and the modality in which they receive the time series data.

We uncover several key insights: common assumptions about LLMs' understanding of time series data are not always accurate, different families of LLMs exhibit varying levels of comprehension, and LLMs show preferences for certain types of time series anomalies. Our work represents the first systematic examination of large language models' anomaly detection capabilities in time series data.


We look into the black box of LLM-based time series analysis methods by focusing on the often overlooked time series anomaly detection task. After a series of ablation studies, we find that while LLM can ``understand'' simple time series anomalies, their ability to understand is highly relevant to their reasoning power and the modality they receive the time series. We find that some common assumptions on how LLM understand time series data are not true, different family of LLMs have different understanding of time series data, and LLMs have a preference for certain types of time series anomalies. Our work is the first to systematically examine large language models' anomaly detection ability on time series data. This work suggests that while using LLMs for analyzing time series is well motivated, they may not be as interpretable as they seem.



Additionally, we introduce a new benchmark, TimeSeriesAD, for evaluating the text-based and visually grounded time series pattern understanding ability of LLMs.




explore time series encoders and reveal that patching and attention structures perform similarly to state-of-the-art LLM-based forecasters.



we derive some insights from this observation.





However, 



We also find that despite their significant computational cost, pretrained LLMs do no better than models trained from scratch, do not represent the sequential dependencies in time series, and do not assist in few-shot settings. Additionally, we explore time series encoders and reveal that patching and attention structures perform similarly to state-of-the-art LLM-based forecasters.



and their math knowledge can be transferred to time series forecasting tasks










are ablated and the results show that removing the LLM component or replacing it with a basic attention layer does not degrade the forecasting results.





Large language models (LLMs) are being applied to time series tasks, particularly time series forecasting. However, are language models actually useful for time series? After a series of ablation studies on three recent and popular LLM-based time series forecasting methods, we find that removing the LLM component or replacing it with a basic attention layer does not degrade the forecasting results—in most cases the results even improved. We also find that despite their significant computational cost, pretrained LLMs do no better than models trained from scratch, do not represent the sequential dependencies in time series, and do not assist in few-shot settings. Additionally, we explore time series encoders and reveal that patching and attention structures perform similarly to state-of-the-art LLM-based forecasters.

Recently, there has been a surge of Transformer-based solutions for the long-term time series forecasting (LTSF) task. Despite the growing performance over the past few years, we question the validity of this line of research in this work. Speciﬁcally, Transformers is arguably the most successful solution to extract the semantic correlations among the elements in a long sequence. However, in time series modeling, we are to extract the temporal relations in an ordered set of continuous points. While employing positional encoding and using tokens to embed sub-series in Transformers facilitate preserving some ordering information, the nature of the permutation-invariant self-attention mechanism inevitably results in temporal information loss.

To validate our claim, we introduce a set of embarrassingly simple one-layer linear models named LTSF-Linear for comparison. Experimental results on nine real-life datasets show that LTSF-Linear surprisingly outperforms existing sophisticated Transformer-based LTSF models in all cases, and often by a large margin. Moreover, we conduct comprehensive empirical studies to explore the impacts of various design elements of LTSF models on their temporal relation extraction capability. We hope this surprising ﬁnding opens up new research directions for the LTSF task. We also advocate revisiting the validity of Transformer-based solutions for other time series analysis tasks (e.g., anomaly detection) in the future. Code is available at: https://github.com/cure-lab/LTSFLinear.

Time series anomaly detection has been a perennially important topic in data science, with papers dating back to the 1950s. However, in recent years there has been an explosion of interest in this topic, much of it driven by the success of de ep learning in other domains and for other time series tasks. Most of these papers test on one or more of a handful of popular benchmark datasets, created by Yahoo, Numenta, NASA, etc. In this work we make a surprising claim. The majority of the individual exemplars in these datasets suffer from one or more of four flaws. Because of these four flaws, we believe that many published comparisons of anomaly detection algorithms may be unreliable, and more importantly, much of the apparent progress in recent years may be illusionary. In addition to demonstrating these claims, with this paper we introduce the UCR Time Series Anomaly Archive. We believe that this resource will perform a similar role as the UCR Time Series Classification Archive, by providing the community with a benchmark that allows meaningful comparisons between approaches and a meaningful gauge of overall progress.

By encoding time series as a string of numerical digits, we can frame time series forecasting as next-token prediction in text. Developing this approach, we find that large language models (LLMs) such as GPT-3 and LLaMA-2 can surprisingly zeroshot extrapolate time series at a level comparable to or exceeding the performance of purpose-built time series models trained on the downstream tasks. To facilitate this performance, we propose procedures for effectively tokenizing time series data and converting discrete distributions over tokens into highly flexible densities over continuous values. We argue the success of LLMs for time series stems from their ability to naturally represent multimodal distributions, in conjunction with biases for simplicity, and repetition, which align with the salient features in many time series, such as repeated seasonal trends. We also show how LLMs can naturally handle missing data without imputation through non-numerical text, accommodate textual side information, and answer questions to help explain predictions. While we find that increasing model size generally improves performance on time series, we show GPT-4 can perform worse than GPT-3 because of how it tokenizes numbers, and poor uncertainty calibration, which is likely the result of alignment interventions such as RLHF.

Time series data are ubiquitous across a wide range of real-world domains. While real-world time series analysis (TSA) requires human experts to integrate numerical series data with multimodal domain-specific knowledge, most existing TSA models rely solely on numerical data, overlooking the significance of information beyond numerical series. This oversight is due to the untapped potential of textual series data and the absence of a comprehensive, high-quality multimodal dataset. To overcome this obstacle, we introduce Time-MMD, the first multi-domain, multimodal time series dataset covering 9 primary data domains. Time-MMD ensures fine-grained modality alignment, eliminates data contamination, and provides high usability. Additionally, we develop MM-TSFlib, the first multimodal time-series forecasting (TSF) library, seamlessly pipelining multimodal TSF evaluations based on Time-MMD for in-depth analyses. Extensive experiments conducted on Time-MMD through MM-TSFlib demonstrate significant performance enhancements by extending unimodal TSF to multimodality, evidenced by over 15\% mean squared error reduction in general, and up to 40\% in domains with rich textual data. More importantly, our datasets and library revolutionize broader applications, impacts, research topics to advance TSA. The dataset and library are available at https://github.com/AdityaLab/Time-MMD and https://github.com/AdityaLab/MM-TSFlib.











